Interpretable and Effective Reinforcement Learning for Attacking against Graph-based Rumor Detection

Social networks are frequently polluted by rumors, which can be detected by advanced models such as graph neural networks. However, the models are vulnerable to attacks and understanding the vulnerabilities is critical to rumor detection in practice. To discover subtle vulnerabilities, we design a powerful attacking algorithm to camouflage rumors in social networks based on reinforcement learning that can interact with and attack any black-box detectors. The environment has exponentially large state spaces, high-order graph dependencies, and delayed noisy rewards, making the state-of-the-art end-to-end approaches difficult to learn features as large learning costs and expressive limitation of graph deep models. Instead, we design domain-specific features to avoid learning features and produce interpretable attack policies. To further speed up policy optimization, we devise: (i) a credit assignment method that decomposes delayed rewards to atomic attacking actions proportional to the their camouflage effects on target rumors; (ii) a time-dependent control variate to reduce reward variance due to large graphs and many attacking steps, supported by the reward variance analysis and a Bayesian analysis of the prediction distribution. On three real world datasets of rumor detection tasks, we demonstrate: (i) the effectiveness of the learned attacking policy compared to rule-based attacks and current end-to-end approaches; (ii) the usefulness of the proposed credit assignment strategy and variance reduction components; (iii) the interpretability of the policy when generating strong attacks via the case study.

==> backup.tex <==
According to Eq.~(\ref{eq:q_objective}), the linear function $\mathbf{x}^\top \bt$ is used to predict the future return starting state-action pair$(s,a)$ by following the policy parameterized by $\bt$.
When the rewards with the baseline $b$ are used for training,
the target variate $r$ is given by the function $\mathbf{x}^\top \bt+ b$ with additive data noise $\epsilon$, i.e. $r=\mathbf{x}^\top \bt+ b+\epsilon$.
The time-dependent baseline could be seen as "clustering" the rewards according to the time $t$. 
It approximates $b$ with Eq.~(\ref{eq:baseline}) and leads to different reward distributions in each time $t$,
so we consider the reward probability distribution $p(r)$ as the mixture model like
\begin{equation}
    \label{eq:mixture}
    p(r) = \sum_t{\lambda_tp(r_t)}
\end{equation}
where $p(r_t)$ is the $t$-th component corresponding to time $t$. The parameter $\lambda_t =1/T$ and $\sum_t{\lambda_t}=1$. 
$\sigma^2$ and $\sigma_t^2$ are the variances of $p(r)$ and $p(r_t)$. 
Compared with no "clustering" reward with the baseline as Eq. (\ref{eq:const_baseline}), it makes sense to reduce the variance intuitively. 
We focus on the expectation of $\sigma_t^2$ to evaluate the variance because the rewards are predicted by the components $p(r_t)$.
It can be proved that $\sigma^2\geq\sum_t{\lambda_t\sigma_t^2}=\mathbb{E}_t[\sigma_t^2]$ and details are shown in Supplementary \ref{app.mixture_v}.
If the empirical average reward values is similar to the mathematical expectation, the "clustering" of rewards could reduce the variance in $r_t$ effectively.
We have $Var(r)\geq \mathbb{E}_t[Var(r_t)]$ with enough training data.
In fact, the state-dependent or action-dependent baseline could also been seen as "clustering" the rewards according to the state or the action. However, it deviates the expectation due to the large state and action spaces. By contrast, the length of horizon has less impact on estimation of the mean, so we regard the time as the "clustering" factor and propose the time-dependent baseline.

\noindent\textbf{Reduced variance in the predicted rewards}.
For the target variate $r=\mathbf{x}^\top \bt+b+\epsilon$, it assumes that $\epsilon$ is zero mean Gaussian noise with the precision (inverse variance) $\beta$,
we show that the reduced variance in the rewards can be transferred to reduced variance in future predictions. 
Using Bayesian ridge regression,
according to Eq. (3.57) and Eq.~(3.58) of \cite{prml},
the predictive distribution $p(r|\mathbf{x},\boldsymbol{r},\boldsymbol{S},\beta)$ at a new input $\bx$
has variance 
\begin{gather}
    \label{eq:pd_variance}
    {\eta}^2(\mathbf{x})=\frac{1}{\beta}+\mathbf{x}^{\top}\boldsymbol{S}\mathbf{x}
    % \\
    % \boldsymbol{S}^{-1}=\boldsymbol{S}^{-1}_0+\beta{\mathbf{X}}^{\top}{\mathbf{X}},
\end{gather}
% $\boldsymbol{S}$ and $\boldsymbol{S}_0$ are variances of the posterior distribution and conjugate prior distribution, respectively.
where $1/\beta=\sigma^2$. $\boldsymbol{S}$ is the variance of the posterior distribution of $N$ observed data. The posterior distribution becomes narrower when new data are observed so the second term goes to zero as $N\rightarrow\infty$ \cite{Qazaz1997}. 
Using maximum likelihood estimation, we can estimate the $\beta$ as in Eq. (3.21) of \cite{prml}:
\begin{equation}
    \label{eq:beta}
    \frac{1}{\tilde{\beta}}=\frac{1}{N}\sum^N_{n=1}{(r_n-\bt^{\top}\mathbf{x}-b)}^2= Var(r)
    % =\textnormal{Var}(r),
\end{equation}
since $\mathbb{E}[r_n]=\bt^\top \bx+b$. 
% $N$ is the number of input training data.
When we construct the distribution of target variate $r$ as the mixture model like Eq.~(\ref{eq:mixture}), the predictive distribution is also a mixture model like
\begin{gather}
    \label{eq:pd_mx_variance}
    p(r|\mathbf{x},\boldsymbol{r},\boldsymbol{S},\beta)=\sum_t{\lambda_t p(r_t|\mathbf{x}_t,\boldsymbol{r}_t,\boldsymbol{S},\beta_t)}, 
\end{gather}
and the the variance of $t$-th component is ${\eta}_t^2(\mathbf{x}_t)$. 
The maximum likelihood of $1/\beta_t$ is
\begin{gather}
    \frac{1}{\tilde{\beta}_t}=\frac{1}{E}\sum^E_{e=1}{(r_t-\bt^{\top}\mathbf{x}_t-b_t)}^2= Var(r_t),
\end{gather}
where $b_t$ is the baseline as Eq.~(\ref{eq:baseline}). $E$ is the number of the training episode and $N=ET$.
Due to $Var(r)\geq \mathbb{E}_t[Var(r_t)]$,
it can be proved that ${\eta}^2(\mathbf{x})\approx 1/\tilde{\beta}  
    \geq \mathbb{E}_t[1/\tilde{\beta}_t] \approx\mathbb{E}_t[{\eta}_t^2(\mathbf{x}_t)]$ with maximum likelihood estimation and $N\rightarrow\infty$. 
The complete proof is shown in Supplementary~\ref{app.mx_PD}.
% \begin{equation}
%     \label{eq:beta}
%     \frac{1}{\tilde{\beta}_{t}}=\frac{1}{N}\sum^N_{n=1}{(r_{n,t}-\bt^{\top}\mathbf{x}_t)}^2=\sigma_t^2.
% \end{equation}
%and the variance of $p(r_t|\mathbf{x}_t,\boldsymbol{r}_t,\boldsymbol{S}_t,\beta_t)$ is ${\eta}_t^2(\mathbf{x}_t)=\frac{1}{\beta_t}+\mathbf{x}_t^{\top}\boldsymbol{S}_t\mathbf{x}_t$.

% A reduced $\textnormal{Var}(r_t)$ directly lead to a reduced variance in the predicted reward in Eq. (\ref{eq:pd_variance}).
% We could not handle the prediction variance directly but it is possible to reduce $1/\beta$ through reducing variance in $r_n$. Thus we achieve the reduction of the overall variance of predictions by reducing $\textnormal{Var}(\tilde{r}_t)$.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.35\textwidth]{acmart-primary/samples/images/graphical_model.pdf}
%     \caption{The random variables in the MDP have the dependencies represented by the graphical model. According to $D$-separation, any path going from $R_t$ to $R_{t+1}$ is blocked by the observed state $S_{t+1}$,
%     so that the two rewards are conditional independent conditioned on $S_{t+1}$.}
%     \label{fig:graphical_model}
% \end{figure}

% \noindent\textbf{Independence of the control variates}.
% $V^\pi(t)$ is defined for each $t$ across trajectories, rather than depending on rewards from other steps in the same trajectory.
% The implicit assumption is that the rewards from different time steps are conditional independent.
% This can be justified by the graphical model in Figure~\ref{fig:graphical_model} and $D$-separation~\cite{prml}.

% \begin{algorithm}
%     \caption{AdRumor-RL \textcolor{red}{Too many functions that are not defined; too many details}}
%     \label{alg:alg}
%     \begin{algorithmic}[1]
%         \Require 
%                 $\alpha$, $E$, $T$,
%                 target model $f$, 
%                 ${\mathcal G}$=$({\mathcal V}$, 
%                 ${\mathcal E})$, ${\mathcal G}_{user}$, 
%                 controllable node set ${\mathcal V}'$, 
%                 controllable edge set ${\mathcal E}'$, 
%                 target rumor set ${\mathcal O}$,
%                 subgraph feature extraction method $\Phi^g$,
%                 node feature extraction method $\Phi^n$,
%                 history training inputs matrix $\mathbf{X}^{g}$ and $\mathbf{X}^{n}$
%         \State $\boldsymbol{w}\gets Calculate Taget Influence(\mathcal G, {\mathcal G}_{user}, \mathcal O)$ Eq. (\ref{eq:inf})
%         \For{$eps=1,2,3,...,E$}
%             \State ${\mathcal G}'\gets\mathcal G$
%             \If{$eps=1$}
%                 \State $\bt^g,\bt^n \gets Initialize()$
%             \EndIf
%             \For{$t=1,2,3,...,T$}
%                 \State $\mathcal{A}_1\gets SubgraphPairActionSpece({\mathcal G}', {\mathcal V}', {\mathcal E}', \mathcal O)$
%                 \ForAll{$(G_i,G_j)\in\mathcal{A}_1$}
%                     \State $\mathbf{x}^{g}_{(i,j)}\gets \Phi^g(G_i)\oplus\Phi^g(G_j)$
%                 \EndFor
%                 \State $(G_i,G_j)\gets ChooseAction(\mathcal{A}_1,{\mathbf{x}^{g}_{(i,j)\in\mathcal{A}_1}},\mathbf{X}^g)$ Eq. (\ref{eq:linucb})
%                 \State $\mathbf{x}^{g}_t\gets \mathbf{x}^{g}_{(i,j)}$
%                 \State $\mathbf{X}^g\gets UpdateMatrix(\mathbf{x}^{g}_t)$
%                 \State $\mathcal{A}_2\gets NodePairActionSpece((G_i,G_j), {\mathcal E}')$
%                 \ForAll{$(v_p,v_q)\in\mathcal{A}_2$}
%                     \State $\mathbf{x}^{n}_{(p,q)}\gets \Phi^n(v_p)\oplus\Phi^n(v_q)$
%                 \EndFor
%                 \State $(v_p,v_q)\gets ChooseAction(\mathcal{A}_2,\mathbf{x}^{n}_{(p,q)\in\mathcal{A}_2},\mathbf{X}^n)$ Eq. (\ref{eq:linucb})
%                 \State $\mathbf{x}^{n}_t\gets \mathbf{x}^{n}_{(p,q)}$
%                 \State $\mathbf{X}^n\gets UpdateMatrix(\mathbf{x}^{n}_t)$
%                 \State ${\mathcal G}' \gets AddEdge({\mathcal G}',(v_p,v_q))$
%                 \State $\tilde{r}_t \gets CalculateReward({f,{\mathcal G}',\boldsymbol{w}})$ Eq. (\ref{eq:new_reward})
%             \EndFor
%             % \State Update $\bt^g$ and $\bt^n$ using Eq. (\ref{eq:asy_update}) with $\mathbf{x}^{g}_t$ and $\mathbf{x}^{n}_t$ respectively
%             \State $\bt^g\gets PolicyUpdate(\{(\mathbf{x}^{g}_t,\tilde{r}_t)|t=1,...,T\})$  Eq. (\ref{eq:theta_update})
%             \State $\bt^n\gets PolicyUpdate(\{(\mathbf{x}^{n}_t,\tilde{r}_t)|t=1,...,T\})$  Eq. (\ref{eq:theta_update})
%         \EndFor
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{AdRumor-RL}
%     \label{alg:alg}
%     \begin{algorithmic}[1]
%         \Require 
%                 $\alpha$, $N$, $T$,
%                 target model $f$, 
%                 ${\mathcal G}$, ${\mathcal G}_{user}$, 
%                 the constraint set $C=\{{\mathcal V}',{\mathcal E}',{\mathcal O}\}$,
%                 feature extraction method $\Phi^g$ and $\Phi^n$
%         \State Calculate messages influence $\boldsymbol{w}$ using Eq. (\ref{eq:inf}) on ${\mathcal G}$ and ${\mathcal G}_{user}$
%         \For{$eps=1,2,3,...,E$}
%             \State Initialize the attack graph ${\mathcal G}'$ with $\mathcal G$
%             \If{$n=1$}
%                 \State Initialize policy parameters $\bt^g$ and $\bt^n$
%             \EndIf
%             \For{$t=1,2,3,...,T$}
%                 \State Obtain subgraph level action space $\mathcal{A}_1$ on ${\mathcal G}'$ with $C$
%                 \State Extract subgraph pair features on $\mathcal{A}_1$ with $\Phi^g$
%                 \State Choose the best subgraph pair $(G_i,G_j)$ using Eq. (\ref{eq:linucb})
%                 \State Save the features of $(G_i,G_j)$ as $\mathbf{x}^{g}_t$
%                 \State Obtain node level action space $\mathcal{A}_2$ on $(G_i,G_j)$ with $C$
%                 \State Extract node pair features on $\mathcal{A}_2$ with $\Phi^n$
%                 \State Choose the best node pair $(v_p,v_q)$ using Eq. (\ref{eq:linucb})
%                 \State Save the features of $(G_i,G_j)$ as $\mathbf{x}^{n}_t$
%                 \State Add the edge $(v_p,v_q)$ in ${\mathcal G}'$
%                 \State Calculate reward $\tilde{r}_t$ using Eq. (\ref{eq:new_reward}) on ${\mathcal G}'$ with $f$ and $\boldsymbol{w}$
%             \EndFor
%             \State Update $\bt^g$ using Eq. (\ref{eq:theta_update}) with a list of $(\mathbf{x}^{g}_t,\tilde{r}_t)$
%             \State Update $\bt^n$ using Eq. (\ref{eq:theta_update}) with a list of $(\mathbf{x}^{n}_t,\tilde{r}_t)$
%         \EndFor
%     \end{algorithmic}
% \end{algorithm}
